Complete Chess Games Enable LLM Become A Chess Master

Large language models (LLM) have shown remarkable abilities in text generation, question answering, language translation, reasoning and many other tasks. It continues to advance rapidly and is becoming increasingly influential in various fields, from technology and business to education and entertainment. Despite LLM's success in multiple areas, its ability to play abstract games, such as chess, is underexplored. Chess-playing requires the language models to output legal and reasonable moves from textual inputs. Here, we propose the Large language model ChessLLM to play full chess games. We transform the game into a textual format with the best move represented in the Forsyth-Edwards Notation. We show that by simply supervised fine-tuning, our model has achieved a professional-level Elo rating of 1788 in matches against the standard Elo-rated Stockfish when permitted to sample 10 times. We further show that data quality is important. Long-round data supervision enjoys a 350 Elo rating improvement over short-round data.

==> app.tex <==
\newpage
\section*{Appendix}
\input{2_related}

\section{The distribution of data}
\label{statss}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{sts.png}
    \vspace{.5em} 
    \caption{The distribution of data. Long round data have a large number of turn rounds.}
    % \vspace{-2em}
    \label{fig:Gameset_stat}
\end{figure}
\section{A sample of data}
\label{datasample}
Figure~\ref{fig:datasample} illustrates the composition format of the data in our dataset.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\textwidth]{datasample.png}
    % \vspace{-1em}
    \caption{One example of training data.}
    % \vspace{-2em}
    \label{fig:datasample}
\end{figure}
\section{Implementation details}
\label{Implement}
We fine-tuned the open-llama 3B model~\cite{openlm2023openllama} using the chess corpus from Section~\ref{sec:dataset}, creating ChessLLM. Specific hyperparameters are in Appendix~\ref{sec:detailtrain}.
We aim to analyze and compare the performance of these two models under varying data usage, detailed in the upcoming evaluation section.

\section{Elo rating}
The Elo rating system~\cite{elo1967proposed} is a method often used in chess to calculate a player's relative skill level. It is named after its creator, Arpad Elo, a Hungarian-born American physics professor and chess enthusiast. This system is used across a variety of competitive games aside from chess, including video games.
The numerical Elo rating of a player represents their expected winning probability against other players. If the high-rated player wins as expected, their rating increase will be modest; On the contrary, if the low-rated player wins, they will gain a substantial increase in their rating, and the high-rated player will also get a significant decrease in their rating.

\section{Detail of general policy}
\label{Gendetail}
To quantify our model's generalization capacity, we integrate the Elo Rating as a metric within the operation task. This evaluation modality, proposed by ChessGPT~\citep{feng2023chessgpt}, assesses the model's ability to distinguish Portable Game Notation (PGN) and associated keywords, subsequently suggesting the most suitable next move at a designated skill level. The model's selection of the upcoming legal move is attributed to a moving score, normalized based on the victory ratio ascertained in the original dataset. 
Notably, our model greatly exceeded the performance of random strategies (approximately 50\%), with Elo Ratings corresponding to relatively high skill levels among human chess players. Due to the difference in input methods of various models, we adapt the input to conform to each model's input space. The evaluation data we use is proposed by ChessGPT. Note our model only generates the best moves, giving it a significant advantage in this task. Given that ChessGPT's training approach is to select from various strategies, similar to a classification problem, and our method is to directly generate the corresponding move, we set our model's accuracy evaluation method as generating a single move choice. If the choice is not available in the following options, a second generation is performed, with a sampling frequency of 10 times. If the outcome cannot be selected after 10 attempts, it is deemed an error.

\section{Different Chess Formats}
\subsection{Universal Chess Interface}
The Universal Chess Interface (UCI) format represents a prevalent method for facilitating communication between chess engines and user interfaces. It manifests chess maneuvers by consolidating the initial and terminal squares of a piece, as evident in the representation "e2e4", implying the movement of pawn from e2 to e4. An illustration of UCI notation for a comprehensive game can be as follows:
\begin{tcolorbox}
1. e2e4 e7e5     
\ 2. Ng1f3 Nb8c6   
3. Bf1b5 a7a6     
\ \ \ 4. Bb5a4 Ng8f6
5. O-O b7b5    
\ \ \ \ 6. Ba4b3 Bf8e7 

7. c2c3 O-O
\ 8. d2d4\ \ \  d7d6 
\ \ \ 9. Rf1e1 Nc6a5  
10. Nb1d2 c7c5 
11. d4d5 Na5c4 
12. Nd2xc4 b5xc4 
\end{tcolorbox}

\subsection{Standard Algebraic Notation}
The Standard Algebraic Notation (SAN) is the official method for recording and describing the moves in a game of international chess. Developed for ease of understanding and efficiency, SAN uses a single letter to represent each piece, excluding pawns, with 'K' for the king, 'Q' for the queen, 'R' for the rook, 'B' for the bishop, and 'N' for the knight. The squares are identified by their file (a-h) and rank (1-8), with the file letter preceding the rank number. When a piece makes a move, SAN notation combines the piece's letter with the square it moves to, such as 'Bg5', indicating a bishop moving to the g5 square. Pawns are denoted by the absence of a letter but include capture notation and promotion information when applicable. Additional notations are used for special moves like castling, checks, and checkmates, making SAN a comprehensive yet concise system for documenting chess gameplay.


\subsection{Portable Game Notation}
The Portable Game Notation (PGN) is a widespread and standard format for recording chess games, which combines the move text with additional metadata to provide a comprehensive record of a chess game. PGN is structured to be both human-readable and machine-readable, designed to facilitate the sharing and analysis of chess games. Each game in PGN begins with a set of tag pairs that encapsulate the game's metadata, such as event, site, date, players, and game outcome. The moves of the chess game follow this header section in Standard Algebraic Notation (SAN), complete with annotations and commentary enclosed in curly or semicolon brackets for deeper insights into strategic gameplay. The effectiveness of PGN is exemplified by its universal adoption, serving as the de facto standard for chess software, databases, and online platforms involved in the curation, discussion, and dissemination of chess games at all levels.

\begin{tcolorbox}

[Event ``World Chess Championship'']
    
[Site ``New York, USA'']

[Date ``2024.2.1'']

[Round ``1'']

[White ``Carlsen, Magnus'']

[Black ``Nepo, Ian'']

[Result ``1/2-1/2'']

1. e4 e5 2. Nf3 Nc6 3. Bb5 a6 4. Ba4 Nf6 5. O-O Be7 6. Re1 b5 7. Bb3 d6 8. c3 O-O 9. h3 Nb8 10. d4 Nbd7 11. Nbd2 Bb7 12. Bc2 Re8 13. Nf1 Bf8 14. Ng3 g6 15. a4 c5 16. d5 c4 17. Be3 Qc7 18. Qd2 Nc5 19. Bh6 Be7 20. Nh2 Nfd7 21. Rf1 bxa4 22. Bxa4 Nxa4 23. Rxa4 a5 24. f4 exf4 25. Qxf4 Ne5 26. Ng4 Bd8 27. Bg5 Bxg5 28. Qxg5 Nxg4 29. hxg4 Re5 30. Nf5 Rae8 31. Nh6+ Kg7 32. Qf6+ Kxh6 33. Rf3 Qc5+ 34. Kh1 Rh5+ 35. gxh5 Rxe4 36. Ra1 Qxd5 37. hxg6 Rh4+ 38. Qxh4+ Kxg6 39. Rf6+ Kg7 40. Qh6+ Kg8 41. Rf3 f5 42. Rg3+ Kf7 43. Rg7+ Ke8 44. Re1+ Kd8 45. Qf6+ Kc8 46. Qf8\# 1-0

\end{tcolorbox}

\subsection{Forsyth-Edwards Notation}
The Forsyth-Edwards Notation (FEN) is a standard notation for describing a particular board position of a chess game. The utility of FEN lies in its ability to provide a concise and unambiguous representation of the game state at any given turn, without the need to outline previous moves or strategies. A FEN record consists of six fields which depict the placement of pieces, the active color, castling availability, en passant target square, halfmove clock, and fullmove number. The piece placement field compactly details the specific arrangement of pieces on the board, using a single letter for each chess piece and numbers to denote empty squares, all interleaved by slashes that signify row demarcations from the 8th to the 1st rank. This informative snapshot is integral for the analysis, reconstruction, and continuation of chess games from any halted state, making FEN an indispensable tool for chess enthusiasts, publishers, and digital platforms that facilitate the study and exchange of intricate chess endgames and problems.

\begin{tcolorbox}
    rnbqkbnr/pppppppp/8/8/8/8/\\PPPPPPPP/RNBQKBNR w KQkq - 0 1
\end{tcolorbox}

\section{Why we chose FEN?}
We have selected the Forsyth-Edwards Notation (FEN) to represent the current position on the chessboard for the following reasons. First and foremost, human chess players do not rely on memory regarding past game moves. Instead, as an amateur player typically operates, the focus is on contemplating the next move based solely on the current position. Furthermore, while the Universal Chess Interface (UCI) or Portable Game Notation (PGN) formats utilized by ChessGPT may represent 50 moves of gameplay using approximately 512 tokens—and this number rises linearly as more moves are made—the FEN format maintains a relatively constant token length across different board positions, requiring around 50 tokens. Consequently, employing FEN for chess aligns more closely with the human approach to the game. 
From a machine learning and data generation standpoint:
\begin{itemize}

\item Token Efficiency: The FEN's fixed token length is advantageous because it facilitates easier batching of data for training since each instance is the same size, potentially reducing padding and waste during training.
\item Memory and Storage Considerations: With a FEN representation, data storage becomes more efficient. Since FEN strings have a consistent length, they are more predictable and manageable in terms of memory allocation within databases or while in transit across networks.
\item Computational Performance: Processing FEN strings is less computationally intensive compared to parsing full PGNs especially when you need to quickly generate large datasets or require faster inference times.
\item Training Data Bias: Using FEN as a means for generating training data mitigates the risk of biasing the model towards the most frequently occurring openings or positions found in long PGNs. It allows for a more uniform representation of diverse positions, which is crucial for the generality and robustness of a chess-playing algorithm.
\end{itemize}
\begin{table}[htbp]
    \tiny
    \centering
    \caption{ChessLLM Training Hyperparameters}
    % \vspace{-1em}
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{lrlrlr}
\toprule
Hyperparameters & Value \\\hline
Learning Rate & 1e-4 \\
Warmup Step & 0 \\
Weight decay & 1e-6 \\
Batch Size Per GPU & 100 \\
Number of GPUs & 8*A100 80G\\
Optimizer & Adamw \\
Optimizer beta1 & 0.9 \\
Optimizer beta2 & 0.95 \\
Optimizer epsilon & 1e-9 \\
Precision & AMP \\
Learning Rate Scheduler & Cosine \\
Epochs & 2\\\bottomrule
    \end{tabular}
    }
    \label{tab:pama}
    % \vspace{-3.5em}
\end{table}

\section{Compute resources}
\subsection{Dataset construction resources}
We deployed a computational effort utilizing 4,800 CPU cores based on the Intel(R) Xeon(R) Platinum 8336C CPU @ 2.30GHz, executing a search duration totaling 170 hours.

\subsection{Training resources}
We use 8 $\times$ 80G A100 GPUs for all our experiments. It takes 160 hours to train ChessLLM.

\section{Sample a game with ChessLLM \& Stockfish}



\section{Copyright}
Our data utilization adheres to the stipulations of the GPLv2 license as employed by ChessDB, ensuring compliance with the prescribed guidelines.

Figure~\ref{fig:match} show a match between ChessLLM and Stockfish.
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{match.png}
    % \vspace{-2em}
    \caption{ChessLLM with white chess beat Stockfish at skill level 1. We only include the opening and endgame phases.}
    \label{fig:match}
    % \vspace{-1.5em}
\end{figure*}
\section{ChessLLM Training Details}
\label{sec:detailtrain}
Table~\ref{tab:pama} show details of our training.
